Collaborative knowledge exchange promotes innovation

Considering collaborative patent development, we provide micro-level evidence for innovation through exchanges of differentiated knowledge. Knowledge embodied in a patent is proxied by word pairs appearing in its abstract, while novelty is measured by the frequency with which these word pairs have appeared in past patents. Inventors are assumed to possess the knowledge associated with patents in which they have previously participated. We find that collaboration by inventors with more mutually differentiated knowledge sets is likely to result in patents with higher novelty.

==> latexmkrc <==


add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        #system( "latexmk -cd -pdf #\"$_[0]\"" );

        #FOR XELATEX
        system( "latexmk -cd -xelatex \"$_[0]\"" );

   }
}

#END { system('cp', 'output.bbl', #'main.bbl'); }
